Branch and Price for the Length-Constrained Cycle Partition Problem

The length-constrained cycle partition problem (LCCP) is a graph optimization problem in which a set of nodes must be partitioned into a minimum number of cycles. Every node is associated with a critical time and the length of every cycle must not exceed the critical time of any node in the cycle. We formulate LCCP as a set partitioning model and solve it using an exact branch-and-price approach. We use a dynamic programming-based pricing algorithm to generate improving cycles, exploiting the particular structure of the pricing problem for efficient bidirectional search and symmetry breaking. Computational results show that the LP relaxation of the set partitioning model produces strong dual bounds and our branch-and-price method improves significantly over the state of the art. It is able to solve closed instances in a fraction of the previously needed time and closes 13 previously unsolved instances, one of which has 76 nodes, a notable improvement over the previous limit of 52 nodes.

==> cg.tex <==
\mg{can we call it background if we're introducing also the pricing problem specific to LCCP?}
\mg{Move problem specific notation to sec 3 and the background part in introduction}
Column generation is an advanced technique for
solving combinatorial optimization problems.
Dating back to $1951$~\cite{uchoa_kantorovich_nodate}, it has since been especially effective at solving vehicle routing problems (see \cite{costa_exact_2019} for a survey).
Branch-and-price is a technique for solving optimization problems with a large number of variables. It is an algorithm based on branch-and-bound \cite{}, where each of the subproblems LP-relaxation is solved using column generation \cite{}.
\el{I think this paragraph needs a bit of work. You could get pedantic reviewers these kinds of general statements. Col gen is for solving LPs, therefore not ``combinatorial'' in the general case.}

The \emph{linear programming} (LP) relaxation of \eqref{IMP} is called the \emph{master problem} (MP).
% \begin{equation}
% 	\begin{array}{lll}
% 		\min & \sum_{r \in \Omega} \lambda_r & \\\\
% 		s.t. & \sum_{r \in \Omega} a_i^r  \lambda_r = 1, \quad \forall  i \in V, \quad (\pi_i) \\\\
% 		  & \lambda_{r} \geq 0, \quad\quad\quad\quad\quad \forall{r \in \Omega}.
% 	\end{array}
% 	\tag{MP}
% 	\label{MP}
% \end{equation}
It can solved using column generation.
% \el{You need to be careful with picky reviewers here. I sometimes get them. }
Replace $\Omega$ with a subset of columns $\Omega' \subset \Omega$, forming a \emph{restricted master problem} (RMP).
Column generation first optimizes the RMP, producing a primal-dual~$(\lambda, \pi)$ pair of solutions.
A \emph{pricing problem} is then solved to find improving columns.
If no improving column can be added to~$\Omega'$, then~$\lambda$ is an optimal solution of \eqref{MP}. Otherwise, the improving columns are added to the RMP and the process is repeated.

% MG: Not sure if this equation adds anything extra
% Given a set of cycles~$\Omega'$ that would ideally allow for a feasible solution, we initialize the model yielding a \emph{restricted
% master problem}.

% \begin{equation}
% 	\begin{array}{lll}
% 		\min & \sum_{r \in \Omega'} \lambda_r & \\\\
% 		s.t. & \sum_{r \in \Omega'} a_i^r  \lambda_r = 1, \quad \forall  i \in C, \\\\
% 		  & \lambda_{r} \geq 0, \quad\quad\quad\quad\quad \forall{r \in \Omega'}.
% 	\end{array}
% 	\tag{RMP}
% \end{equation}

An improving column is a column with a negative reduced cost.
Given a dual solution~$\pi \in R^{|C|}$.
\el{I'm a bit confused here. You wrote $C$ to mean the set of nodes previously but I thought it was a typo for $V$.}
The reduced cost of a column can be computed
by~$\overline{c}_r = 1 - \Sigma_{i \in C} a^r_i \pi_i$,
where the first term is true cost of the column, and the second term is the sum of duals for
\el{Better to put a constraint/equation number} the nodes in the column's cycle.

The problem of finding the best improving column, i.e., the one with the minimum reduced cost, is called the
\emph{pricing problem}.
For the LCCP, the pricing problem is
\begin{equation}
	\begin{array}{lll}
		\underset{r \in \Omega}{\text{argmin}} & 1 -  \sum_{i \in r} \pi_i.  & \\
	\end{array}
	\tag{PP}
	\label{PP}
\end{equation}

Due to the large size of the set~$\Omega$ this problem is best solved using an implicit enumeration scheme, such as dynamic programming, which we discuss in the next section.


